Self-Organizing Maps with Variable Input Length for Motif Discovery and Word Segmentation

Time Series Motif Discovery (TSMD) is defined as searching for patterns that are previously unknown and appear with a given frequency in time series. Another problem strongly related with TSMD is Word Segmentation. This problem has received much attention from the community that studies early language acquisition in babies and toddlers. The development of biologically plausible models for word segmentation could greatly advance this field. Therefore, in this article, we propose the Variable Input Length Map (VILMAP) for Motif Discovery and Word Segmentation. The model is based on the Self-Organizing Maps and can identify Motifs with different lengths in time series. In our experiments, we show that VILMAP presents good results in finding Motifs in a standard Motif discovery dataset and can avoid catastrophic forgetting when trained with datasets with increasing values of input size. We also show that VILMAP achieves results similar or superior to other methods in the literature developed for the task of word segmentation.

==> algorithm/update_node_dimension.tex <==
\begin{algorithm}
  	\DontPrintSemicolon
  	\SetKwFunction{Fund}{updateNodeDimension}
	\SetKwInOut{Input}{input}\SetKwInOut{Output}{output}
	\Input{The winner node \boldmath$j$ and the current input pattern \boldmath$x$.}
	\Output{The winner node \boldmath$j$ with your dimension updated.}
    
  	\SetKwProg{Pn}{Function}{:}{\KwRet}
  	\Pn{\Fund{$s$, $x$}}{
      Increase the size of the distance vector \boldmath${ \delta }_{ j }$ until it is the same size as the input pattern \textbf{x};\;
      The new part of the vector \boldmath${ \delta }_{ j }$ is filled with the value 0.0;\;
      Increase the size of the relevance vector \boldmath${ \omega }_{ j }$ until it is the same size as the input pattern \textbf{x};\;
      The new part of the vector \boldmath${ \omega }_{ j }$ is filled with the value 0.5;\;
      Increase the size of the weight vector \boldmath${ c }_{ j }$ until it is the same size as the input pattern \textbf{x};\;
      In the respective positions, the new part of the vector \boldmath${ c }_{ j }$ is filled with the same values of the input pattern \textbf{x};\;
      
  	}
\caption{Update Dimension Node}
\label{alg:updateNodeDimension}
\end{algorithm} 


==> table/gunpoint.tex <==
\begin{table}[!ht]
\centering
\caption{Gun-Point dataset characteristics}
\label{table:gunpoint}
\begin{tabular}{ccccc}
\specialrule{.1em}{.05em}{.05em} 
Train Size & Test Size & Length & Number of classes & Type \\ \hline
    50     &   150     & 150    &          2        & Motion \\
 \specialrule{.1em}{.05em}{.05em} 
\end{tabular}
\end{table}
